Compressed Diffusion

Diffusion maps are a commonly used kernel-based method for manifold learning, which can reveal intrinsic structures in data and embed them in low dimensions. However, as with most kernel methods, its implementation requires a heavy computational load, reaching up to cubic complexity in the number of data points. This limits its usability in modern data analysis. Here, we present a new approach to computing the diffusion geometry, and related embeddings, from a compressed diffusion process between data regions rather than data points. Our construction is based on an adaptation of the previously proposed measure-based Gaussian correlation (MGC) kernel that robustly captures the local geometry around data points. We use this MGC kernel to efficiently compress diffusion relations from pointwise to data region resolution. Finally, a spectral embedding of the data regions provides coordinates that are used to interpolate and approximate the pointwise diffusion map embedding of data. We analyze theoretical connections between our construction and the original diffusion geometry of diffusion maps, and demonstrate the utility of our method in analyzing big datasets, where it outperforms competing approaches.

==> old-sections/mgc.tex <==
% We consider a diffusion process defined over a dataset $X$.  This process reveals the low dimensional geometry in data by propagating a random walk over local neighborhoods learned via a kernel function.  Let $g(x,y) : \mathbb{R}^M \times \mathbb{R}^M \mapsto \mathbb{R}$ be a kernel function applied over a dataset $X$.  For purposes of clarity, assume that all unspecified integrals are performed over $X$.  The \textit{degree} of the kernel for a point $x$ in a dataset $X$ is given by 
% \begin{align}
% q(x) \triangleq \int g(x,z) dz.
% \label{eqn:qx_degrees}
% \end{align}
% We define the \textit{measure-based diffusion kernel} from [cite] as
% \begin{align}
% k(x,y) \triangleq \int g(x,r) g(r,y) d \mu(r).
% \label{eqn:basic_mgc}
% \end{align}

We use a sparsity measure $d\mu(x) = q^{-1}(x)dx$ to define an MGC kernel
\begin{align}
k_c(x,y) \triangleq \int \frac{g(x,r) g(r,y)}{q(r)} d r.
\label{eqn:compressed_kernel}
\end{align}
This kernel construction will compress the evolution of a diffusion process defined on data.  The compressed kernel emits the degree function $\nu(x) = \int k_c(x,y) dy$.  We begin our analysis by focusing on this notion of degrees in the following proposition.

\begin{proposition}[Volume preservation]
For the compressed diffusion kernel $k_c(x,y)$, $$\nu(x) = q(x).$$ \label{prop:volume_preservation}
\end{proposition}
\begin{proof}
\begin{align*}
    \nu(x) &= \int k_c(x,y) dy = \int \int g(x,r) q(r)^{-1} g(r,y)dr dy \\
        &= \int  g(x,r) q(r)^{-1} \underbrace{\int g(r,y) dy}_{q(r)} dr \\
        &= \int  g(x,r) dr \\
        &= q(x).
\end{align*}
\end{proof}
Next, define the diffusion transition probabilities kernel as $p_c(x,y) \triangleq k_c(x,y)/\nu(x)$.  The associated compressed diffusion operator $P_c: L^2(\mathbb{R}^M) \mapsto L^2(\mathbb{R}^M)$ is defined as
\begin{align}
P_cf(x) \triangleq \int p_c(x,y) f(y)dy.
\label{eqn:compressed_operator}
\end{align}
The uncompressed operator is defined analogously as $Pf(x) \triangleq \int p(x,y)f(y)dy$, where $p(x,y) \triangleq g(x,y)/q(x)$ is the uncompressed transition kernel. These operators yield the following corollary.
\begin{corollary}[Compressed equivalence]
$$P_c f(x) = P^2 f(x)$$
\end{corollary}
\begin{proof}
\begin{align*}
    P_cf(x) &= \int p_c(x,y) f(y)dy = \nu(x)^{-1} \int k(x,y) f(y) dy \\
    &= q(x)^{-1} \int \int g(x,r) q(r)^{-1} g(r,y) dr f(y) dy \\
    &= q(x)^{-1} \int \frac{g(x,r)}{q(r)} \int g(r,y) f(y) dy dr = P^2 f(x)
\end{align*}
\end{proof}

The compressed diffusion kernel is naturally amenable to partition-based coarsening - in this scheme, an assignment function groups data points based on their manifold localization.  In section \ref{sec:partitions} we discuss the selection of these functions.  Defining $S,T \subset X$, we have the \textit{coarsened kernel} 
\begin{align}
    k_L(S,T) \triangleq \int_S\int_T k_c(x,y) dxdy 
    \label{eqn:coarsened_kernel}
\end{align}
The coarsened kernel is also volume preserving.
\begin{proposition}[Volume preservation]
For the coarsened kernel $k_L(S,T)$, $$\nu(S) = \int_S q(x) dx.$$ \label{prop:volume_preservation_coarsening}
\end{proposition}
\begin{proof}
\begin{align*}
    \nu(S) &= \int k_L(S,T) dT \\ 
    &= \iint \left[\int_S g(x,r)dx \right]\left[\int_Tg(r,y)dy \right] q(r)^{-1} dr \,\, dT \\
    &= \int \left[\int_S g(x,r)dx \right] \left[ \iint_T g(r,y)dy \,\, dT \right] q(r)^{-1} dr \\
    &= \int \left[\int_S g(x,r)dx \right] \left[ \int g(r,y)dy \right] q(r)^{-1} dr \\
    &= \iint_S g(x,r) dx\,\, q(r) q^{-1}(r) dr \\ 
    &= \iint_S g(x,r) dx\,\,  dr \\
    &= \int_S \int g(x,r) dr\,\,  dx = \int_S q(x) dx
\end{align*}
\end{proof}

==> old-sections/partitions.tex <==
By design, the landmark kernel should be as close as possible an approximation to the original kernel for the purposes of diffusion. We note that the kernel function $k_L$ defines an affinity between clusters; it is desirable, then, that we choose the assignment function such that $k_L$ shares the properties of the kernel function $g$. Notably, for a radial basis kernel, we have

$$g(x,y) = h( \Vert x - y \Vert )$$

where 

$$h : \mathbb{R} \to [0, \infty) \text{ and } \argmax_{d} h(d) = 0.$$

We seek, then, to choose an assignment function such that we maximize the self-affinity $\sum_S k_L(S,S)$. This is equivalent to solving the \textit{mincut} problem as defined in \textcolor{red}{cite}. However, for practical reasons defined in \textcolor{red}{cite}, we use normalized spectral clustering to minimize a relaxed version of \textit{Ncut} \textcolor{red}{cite}.

Further, we note that since spectral clustering involves singular value decomposition of the kernel matrix, the exact calculation of the coarsened kernel has the same computational complexity as the diffusion map. While this has some advantages for applications which further process the kernel \textcolor{red}{cite PHATE, diffusion t-SNE}, in order to obtain a useful approximation of the diffusion map in the general case we require an assignment function which is linear in the number of points. Here we use KMeans++ \textcolor{red}{cite} as an approximation of spectral clustering, noting that for $k$ sufficiently large, the only Euclidean distances contributing to cluster assignment are small, and hence the non-linearities typically considered a weakness of KMeans that is resolved by spectral clustering \textcolor{red}{cite} tend not to be relevant.
